Statistical Estimation: From Denoising to Sparse Regression and Hidden Cliques

These notes review six lectures given by Prof. Andrea Montanari on the topic of statistical estimation for linear models. The first two lectures cover the principles of signal recovery from linear measurements in terms of minimax risk. Subsequent lectures demonstrate the application of these principles to several practical problems in science and engineering. Specifically, these topics include denoising of error-laden signals, recovery of compressively sensed signals, reconstruction of low-rank matrices, and also the discovery of hidden cliques within large networks.

==> Makefile <==
FILENAME = montanari_lecture
PS_FILE = $(FILENAME).ps
PDF_FILE = $(FILENAME).pdf
LOG_FILE = $(FILENAME).log

PAPERSIZE = a4
# PAPERSIZE = letter

LATEX_FILES = *.dvi *.log *.toc *.tof *.aux *.blg *.lof *.lot *.bbl *.idx *.ind *.ilg
CLEAN_FILES = $(LATEX_FILES) *.bak core $(PS_FILE) $(PDF_FILE) *.out bibbuild.log warnings.log
COMPRESS_FILES = *.tex *.bib *.sty *.eps *.ps *.fig *.m *.txt *.pgm *.bst *.cls
UNCOMPRESS_FILES = *.Z *.gz

COMPRESS_DIRS = . ChapAmin ChapGamarnik ChapMezard ChapMontanari ChapMoore ChapOpper ChapParisi ChapShah ChapZecchina ChapUrbanke
COMPRESS = gzip -q
UNCOMPRESS = gunzip

all: main


main:
	pdflatex -jobname $(FILENAME) main
	bibtex $(FILENAME) >> bibbuild.log
	pdflatex -jobname $(FILENAME) main | grep Warning: > warnings.log
	pdflatex -jobname $(FILENAME) main | grep Warning: > warnings.log
	cp montanari_lecture.bbl ChapMontanari/references.bbl

arxiv: main
	cp montanari_lecture.bbl main.bbl
	rm montanari_lecture.bbl
	rm montanari_lecture.pdf
	rm *.log
	rm *.aux
	rm *.blg
	rm *.out
	rm *.toc

test:
	pdflatex -jobname $(FILENAME) main
	makeindex -p 1 $(FILENAME)
	find . -regex ".*\main.aux" | while read auxfoile; \
	do \
		if grep citation $$auxfile; then bibtex $$auxfile; fi; \
	done
	@while grep Rerun $(LOG_FILE); \
	do \
		pdflatex -jobname LesHouches main; \
		makeindex $(FILENAME);\
		pdflatex -jobname LesHouches main; \
	done


noref:
	pdflatex -jobname $(FILENAME) main
	pdflatex -jobname $(FILENAME) main

view: main
	open $(PDF_FILE)

clean:
	@for i in $(COMPRESS_DIRS) ; \
	do \
	(if (test -d $$i) ; \
	then cd $$i ; \
	echo "Cleaning $$i" ; \
	rm -f *~ ; \
	rm -f $(CLEAN_FILES) ; \
	fi) \
	done

compress: clean
	@for i in $(COMPRESS_DIRS) ; \
	do \
	(if (test -d $$i) ; \
	then cd $$i ; \
	echo "Compressing files in $$i" ; \
	for j in $(COMPRESS_FILES) ; \
	do \
	(if (test -f $$j) ; \
	then $(COMPRESS) $$j ; \
	fi) \
	done ; \
	fi) \
	done

uncompress:
	@for i in $(COMPRESS_DIRS) ; \
	do \
	(if (test -d $$i) ; \
	then cd $$i ; \
	echo Uncompressing files in $$i ; \
	for j in $(UNCOMPRESS_FILES) ; \
	do \
	(if (test -f $$j) ; \
	then $(UNCOMPRESS) $$j ; \
	fi) \
	done ; \
	fi) \
	done

